Coding for Sensing: An Improved Scheme for Integrated Sensing and Communication over MACs

A memoryless state-dependent multiple-access channel (MAC) is considered, where two transmitters wish to convey their messages to a single receiver while simultaneously sensing (estimating) the respective states via generalized feedbacks. For this channel, an improved inner bound is provided on the fundamental rate-distortions tradeoff which characterizes the communication rates the transmitters can achieve while simultaneously ensuring that their state-estimates satisfy desired distortion criteria. The new inner bound is based on a scheme where each transmitter codes over the generalized feedback so as to improve the state estimation at the other transmitter. This is in contrast to the schemes proposed for point-to-point and broadcast channels where coding is used only for the transmission of messages and the optimal estimators operate on a symbol-by-symbol basis on the sequences of channel inputs and feedback outputs.

==> main_v2.bib.tex <==
@string{bellsyst = "Bell Syst. Tech. J."}
@string{it = "IEEE Trans. Info. Theory"}
@string{jsac = "IEEE J. Sel. Areas Commun."}
@string{sig = "IEEE Trans. Signal Process."}
@string{tcom = "IEEE Trans. Commun."}
@string{twc = "IEEE Trans. Wireless Commun."}
@string{veh = "IEEE Trans. Veh. Technol."}
@string{mveh = "IEEE Veh. Technol. Mag. "}
@string{mcom = "IEEE Commun. Mag."}
@string{proc = "Proc. IEEE"}
@string{msig = "IEEE Signal Process. Mag."}
@STRING{allerton= "Proc. Allerton Conf. Communication, Control and Computing"}
@STRING{asilomar = "Proc. Asilomar Conf. Signals, Systems and Computers"}
@STRING{globecom= "Proc. {IEEE} Global Conf. Communications {(GLOBECOM)}"}
@STRING{ICASSP = "Proc. {IEEE} Int. Conf. Acoustics, Speech, and Signal Processing {(ICASSP)}"}
@STRING{ICC = "Proc. {IEEE} Int. Conf. Communications {(ICC)}"}
@STRING{ISIT = "Proc. {IEEE} Int. Symp. Info. Theory {(ISIT)}"}
@STRING{ITA = "Proc. Info. Theory and App. Workshop {(ITA)}"}
@STRING{ITW = "Proc. {IEEE} Info. Theory Workshop {(ITW)}"}
@STRING{SPAWC = "Proc. {IEEE} Workshop on Signal Processing Advances in Wireless Communications {(SPAWC)}"}

@article{gastpar2014coding,
  title={Coding schemes and asymptotic capacity for the Gaussian broadcast and interference channels with feedback},
  author={Gastpar, Michael and Lapidoth, Amos and Steinberg, Yossef and Wigger, Michele},
  journal=it,
  volume={60},
  number={1},
  pages={54--71},
  year={2014},
  publisher={IEEE}
}
@inproceedings{he2014capacity,
  title={On the capacity of the fading broadcast channel with state feedback},
  author={He, Chao and Yang, Sheng and Piantanida, Pablo},
  booktitle={2014 6th International Symposium on Communications, Control and Signal Processing (ISCCSP)},
  pages={182--185},
  year={2014},
  organization={IEEE}
}
@article{venkataramanan2013achievable,
  title={An achievable rate region for the broadcast channel with feedback},
  author={Venkataramanan, Ramji and Pradhan, S Sandeep},
  journal=it,
  volume={59},
  number={10},
  pages={6175--6191},
  year={2013},
  publisher={IEEE}
}
@article{DUECK,
	title = {Partial feedback for two-way and broadcast channels},
	journal = {Information and Control},
	volume = {46},
	number = {1},
	pages = {1--15},
	year = {1980},
	issn = {0019--9958},
	author = {G. {Dueck}}
}

@book{richards2014fundamentals,
  title={Fundamentals of radar signal processing, Second edition},
  author={Richards, Mark A},
  year={2014},
  publisher={McGraw-Hill Education}
}

@article{wang2012capacity,
  title={On the capacity of 1-to-$K$ broadcast packet erasure channels with channel output feedback},
  author={Wang, Chih C.},
  journal=it,
  volume={58},
  number={2},
  pages={931--956},
  year={2012},
  publisher={IEEE}
}
@article{gatzianas2013multiuser,
  title={Multiuser broadcast erasure channel with feedback: capacity and algorithms},
  author={Gatzianas, Marios and Georgiadis, Leonidas and Tassiulas, Leandros},
  journal=it,
  volume={59},
  number={9},
  pages={5779--5804},
  year={2013},
  publisher={IEEE}
}

@ARTICLE{shayevitz2012capacity,
	author={O. {Shayevitz} and M. {Wigger}},
	journal=it, 
	title={On the Capacity of the Discrete Memoryless Broadcast Channel With Feedback}, 
	year={2013},
	volume={59},
	number={3},
	pages={1329-1345}
	}

@ARTICLE{liu2022CramerRao,
	author={Liu, Fan and Liu, Ya-Feng and Li, Ang and Masouros, Christos and Eldar, Yonina C.},
	journal={IEEE Transactions on Signal Processing}, 
	title={Cramér-Rao Bound Optimization for Joint Radar-Communication Beamforming}, 
	year={2022},
	volume={70},
	number={},
	pages={240-253},
	doi={10.1109/TSP.2021.3135692}}


@ARTICLE{gaudio2019effectiveness,
  author={L. {Gaudio} and M. {Kobayashi} and G. {Caire} and G. {Colavolpe}},
  journal=twc, 
  title={On the Effectiveness of {OTFS} for Joint Radar Parameter Estimation and Communication}, 
  year={2020},
  volume={19},
  number={9},
  pages={5951--5965}
  }


% OTFS channel estimation 
@article{shen2019channel,
  title={Channel Estimation for Orthogonal Time Frequency Space ({OTFS}) Massive {MIMO}},
  author={Shen, Wenqian and Dai, Linglong and An, Jian-ping and Fan, Pingzhi and Heath, Robert W},
  journal=sig,
  year={2019},
  volume={67},
number={16},
pages={4204-4217},
month={Aug},
  publisher={IEEE}
}
% V2X
@article{chen2017vehicle,
  title={Vehicle-to-everything ({V2X}) services supported by {LTE}-based systems and {5G}},
  author={Chen, Shanzhi and Hu, Jinling and Shi, Yan and Peng, Ying and Fang, Jiayi and Zhao, Rui and Zhao, Li},
  journal={IEEE Communications Standards Magazine},
  volume={1},
  number={2},
  pages={70--76},
  year={2017},
  publisher={IEEE}
}


@article{haas1997time,
  title={A time-frequency well-localized pulse for multiple carrier transmission},
  author={Haas, Ralf and Belfiore, Jean-Claude},
  journal={Wireless personal communications},
  volume={5},
  number={1},
  pages={1--18},
  year={1997},
  publisher={Springer}
}

@article{fodor2019supporting,
  title={Supporting Enhanced Vehicle-to-Everything Services by {LTE} Release 15 Systems},
  author={Fodor, Gabor and Do, Hieu and Ashraf, Shehzad Ali and Blasco, Ricardo and Sun, Wanlu and Belleschi, Marco and Hu, Liang},
  journal={IEEE Communications Standards Magazine},
  volume={3},
  number={1},
  pages={26--33},
  year={2019},
  publisher={IEEE}
}

@article{seo2016lte,
  title={{LTE} evolution for vehicle-to-everything services},
  author={Seo, Hanbyul and Lee, Ki-Dong and Yasukawa, Shinpei and Peng, Ying and Sartori, Philippe},
  journal=mcom,
  volume={54},
  number={6},
  pages={22--28},
  year={2016},
  publisher={IEEE}
}

% Magazine
@ARTICLE{hassanien2019dual,
author={A. {Hassanien} and M. G. {Amin} and E. {Aboutanios} and B. {Himed}},
journal=IEEE_M_SP,
title={Dual-Function Radar Communication Systems: A solution to the spectrum congestion problem},
year={2019},
volume={36},
number={5},
pages={115-126},
month={Sep.}
}


@article{liu2017adaptive,
  title={Adaptive {OFDM} integrated radar and communications waveform design based on information theory},
  author={Liu, Yongjun and Liao, Guisheng and Xu, Jingwei and Yang, Zhiwei and Zhang, Yuhong},
  journal=IEEE_J_COML,
  volume={21},
  number={10},
  pages={2174--2177},
  year={2017},
  publisher={IEEE}
}


% Ottersten's group
@article{mishra2019towards,
  title={Towards millimeter wave joint radar-communications: A signal processing perspective},
  author={K. V. {Mishra} and M. R. {Bhavani Shankar} and V. {Koivunen} and B. {Ottersten} and S. A. {Vorobyov}}, 
  journal=IEEE_M_SP,
  year={2019},
  volume={36},
number={5},
pages={100-114},
month={Sep.}
}

@article{dokhanchi2019mmwave,
  title={A {mmWave} automotive joint radar-communications system},
  author={Dokhanchi, Sayed Hossein and Mysore, Bhavani Shankar and Mishra, Kumar Vijay and Ottersten, Bj{\"o}rn},
  journal=IEEE_J_AES,
  year={2019},
  volume={55},
number={3},
pages={1241-1260},
month={June}
}

@inproceedings{dokhanchi2019adaptive,
  title={Adaptive Waveform Design for Automotive Joint Radar-communications System},
  author={Dokhanchi, S Hossein and Shankar, MR Bhavani and Alaee-Kerahroodi, M and Stifter, T and Ottersten, Bj{\"o}rn},
  booktitle=ICASSP,
  pages={4280--4284},
  year={2019},
  organization={IEEE}
}

% Yonina Eldar's group
@article{muns2017beam,
  title={Beam alignment and tracking for autonomous vehicular communication using {IEEE} 802.11 ad-based radar},
  author={Muns, Guillem Reus and Mishra, Kumar Vijay and Guerra, Carlos Bocanegra and Eldar, Yonnina C and Chowdhury, Kaushik R},
  journal={arXiv preprint arXiv:1712.02453},
  year={2017}
}


@ARTICLE{zheng2019radar,
	author={L. {Zheng} and M. {Lops} and Y. C. {Eldar} and X. {Wang}},
	journal={IEEE Signal Processing Magazine}, 
	title={Radar and Communication Coexistence: An Overview: A Review of Recent Methods}, 
	year={2019},
	volume={36},
	number={5},
	pages={85-99},}


@article{ma2019joint,
  title={Joint Radar-Communications Strategies for Autonomous Vehicles},
  author={Ma, Dingyou and Shlezinger, Nir and Huang, Tianyao and Liu, Yimin and Eldar, Yonina C},
  journal={arXiv preprint arXiv:1909.01729},
  year={2019}
}

% resoure-sharing

% frequency splitting
@inproceedings{bicua2019multicarrier,
  title={Multicarrier Radar-communications Waveform Design for {RF} Convergence and Coexistence},
  author={Bic{\u{a}}, M and Koivunen, V and others},
  booktitle=ICASSP,
  year={2019}
}
% spatial beamforming to separate radar and communications
@article{liu2018mu,
  title={{MU-MIMO} communications with {MIMO} radar: From co-existence to joint transmission},
  author={Liu, Fan and Masouros, Christos and Li, Ang and Sun, Huafei and Hanzo, Lajos},
  journal=IEEE_J_WCOM,
  volume={17},
  number={4},
  pages={2755--2770},
  year={2018},
  publisher={IEEE}
}
%%%%%%%%%%%%%%%%%%%%%%%%
@article{matz2013time,
	author={G. {Matz} and H. {Bolcskei} and F. {Hlawatsch}},
	journal=IEEE_M_SP,
	title={Time-Frequency Foundations of Communications: Concepts and Tools},
	year={2013},
	volume={30},
	number={6},
	pages={87-96},
	keywords={Fourier analysis;signal processing;time-frequency analysis;time-frequency foundations;communication theory;signal analysis;Fourier analysis;infinite wave-trains;auditory sensations;OFDM;Time-frequency analysis;Approximation methods;Scattering;Transfer functions;Receivers},
	doi={10.1109/MSP.2013.2269702},
	ISSN={1053-5888},
	month={Nov},
}

@ARTICLE{sabharwal2014band,
author={A. {Sabharwal} and P. {Schniter} and D. {Guo} and D. W. {Bliss} and S. {Rangarajan} and R. {Wichman}},
journal=IEEE_J_JSAC,
title={In-Band Full-Duplex Wireless: Challenges and Opportunities},
year={2014},
volume={32},
number={9},
pages={1637-1652},
keywords={radio links;radio transceivers;in band full duplex wireless;wireless communication systems;wireless terminal;self interference;Topology;Wireless communication;Radar;Network topology;Interference;Relays;Base stations;Full-duplex;simultaneous transmit and receive;wireless communications},
doi={10.1109/JSAC.2014.2330193},
ISSN={0733-8716},
month={Sep.},}

@article{li2007mimo,
	author={J. {Li} and P. {Stoica}},
	journal=IEEE_M_SP,
	title={{MIMO} Radar with Colocated Antennas},
	year={2007},
	volume={24},
	number={5},
	pages={106-114},
	keywords={antenna phased arrays;MIMO communication;phased array radar;radar antennas;government agencies;parameter estimation;adaptive techniques;direct applicability;identifiability;phased-array counterpart;waveform diversity;colocated antennas;MIMO radar;Radar antennas;MIMO;Adaptive arrays;Transmitting antennas;Receiving antennas;Parameter estimation;Radar imaging;Antenna arrays;Radar applications;Doppler radar},
	doi={10.1109/MSP.2007.904812},
	ISSN={1053-5888},
	month={Sep.},
}

@article{kumari2018ieee,
author={P. {Kumari} and J. {Choi} and N. {González-Prelcic} and R. W. {Heath}},
journal=IEEE_J_VT,
title={{IEEE} 802.11ad-Based Radar: An Approach to Joint Vehicular Communication-Radar System},
year={2018},
volume={67},
number={4},
pages={3012-3027},
doi={10.1109/TVT.2017.2774762},
ISSN={0018-9545},
month={April},}

@inproceedings{nguyen2017delay,
author={D. H. N. {Nguyen} and R. W. {Heath}},
booktitle=ICASSP,
title={Delay and Doppler processing for multi-target detection with {IEEE} 802.11 {OFDM} signaling},
year={2017},
volume={},
number={},
pages={3414-3418},
keywords={delay estimation;Doppler radar;object detection;OFDM modulation;radar detection;road vehicle radar;telecommunication signalling;wireless LAN;Doppler information processing;delay information processing;IEEE 802.11 OFDM signaling;IEEE 802.11p OFDM signaling;IEEE 802.11p short-range communication;IEEE 802.11p DSRC;vehicles to automotive radio detection and ranging functionality;vehicles to automotive radar functionality;estimation of signal parameters via rotational invariance technique;concurrent multitarget detection;velocity estimation;range estimation;probability;OFDM;Radar;Estimation;Frequency estimation;Signal resolution;Time-frequency analysis;IEEE 802.11 Standard;Radar;OFDM;802.11;multi-target detection},
doi={10.1109/ICASSP.2017.7952790},
ISSN={2379-190X},
month={March},}

@article{braun2014ofdm,
  title={{OFDM} Radar Algorithms in Mobile Communication Networks},
  author={Braun, Martin},
  journal={Ph.D. Thesis at Karlsruhe Institute of Technology},
  year={2014}
}

@ARTICLE{sturm2011waveform,
author={C. {Sturm} and W. {Wiesbeck}},
journal=IEEE_J_PROC,
title={Waveform Design and Signal Processing Aspects for Fusion of Wireless Communications and Radar Sensing},
year={2011},
volume={99},
number={7},
pages={1236-1259},
doi={10.1109/JPROC.2011.2131110},
ISSN={0018-9219},
month={July}}


@article{raviteja2018interference,
	author={P. {Raviteja} and K. T. {Phan} and Y. {Hong} and E. {Viterbo}},
	journal=IEEE_J_WCOM,
	title={Interference Cancellation and Iterative Detection for Orthogonal Time Frequency Space Modulation},
	year={2018},
	volume={17},
	number={10},
	pages={6501-6515},
	doi={10.1109/TWC.2018.2860011},
	ISSN={1536-1276},
	month={Oct},
}

@article{li2017simple,
  title={A simple two-stage equalizer with simplified orthogonal time frequency space modulation over rapidly time-varying channels},
  author={Li, Li and Wei, Hua and Huang, Yao and Yao, Yao and Ling, Weiwei and Chen, Gong and Li, Peng and Cai, Yunlong},
  journal={arXiv preprint arXiv:1709.02505},
  year={2017}
}



@ARTICLE{viterboOTFSradar,
       author = {{Raviteja}, P. and {Phan}, Khoa T. and {Hong}, Yi and {Viterbo},
        Emanuele},
        title = {Orthogonal Time Frequency Space ({OTFS}) Modulation Based Radar System},
      journal = {arXiv e-prints},
     keywords = {Computer Science - Information Theory},
         year = 2019,
        month = Jan,
          eid = {arXiv:1901.09300},
        pages = {arXiv:1901.09300},
archivePrefix = {arXiv},
       eprint = {1901.09300},
 primaryClass = {cs.IT},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2019arXiv190109300R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{patole2017automotive,
	author={S. M. {Patole} and M. {Torlak} and D. {Wang} and M. {Ali}},
	journal=IEEE_M_SP,
	title={Automotive radars: A review of signal processing techniques},
	year={2017},
	volume={34},
	number={2},
	pages={22-35},
	doi={10.1109/MSP.2016.2628914},
	ISSN={1053-5888},
	month={March},
}

@book{athley2003space,
  title={Space-time parameter estimation in radar array processing},
  author={Athley, Fredrik},
  year={2003},
  publisher={Department of Signals and Systems, School of Electrical Engineering, Chalmers University of Technology.}
}

@article{athley2005threshold,
	author={F. {Athley}},
	journal=IEEE_J_SP,
	title={Threshold region performance of maximum likelihood direction of arrival estimators},
	year={2005},
	volume={53},
	number={4},
	pages={1359-1373},
	doi={10.1109/TSP.2005.843717},
	ISSN={1053-587X},
	month={April},
}

@ARTICLE{colavolpe2011SISOdetection,
	author={G. {Colavolpe} and D. {Fertonani} and A. {Piemontese}},
	journal=IEEE_J_STSP,
	title={{SISO} Detection Over Linear Channels With Linear Complexity in the Number of Interferers},
	year={2011},
	volume={5},
	number={8},
	pages={1475-1485},
	doi={10.1109/JSTSP.2011.2168943},
	ISSN={1932-4553},
	month={Dec},
}

@article{kavcic2003binary,
	author={A. {Kavcic} and {Xiao Ma} and M. {Mitzenmacher}},
	journal=IEEE_J_IT,
	title={Binary intersymbol interference channels: Gallager codes, density evolution, and code performance bounds},
	year={2003},
	volume={49},
	number={7},
	pages={1636-1652},
	doi={10.1109/TIT.2003.813563},
	ISSN={0018-9448},
	month={July},}
}

@article{soriaga2007determining,
author={J. B. {Soriaga} and H. D. {Pfister} and P. H. {Siegel}},
journal=IEEE_J_IT,
title={Determining and Approaching Achievable Rates of Binary Intersymbol Interference Channels Using Multistage Decoding},
year={2007},
volume={53},
number={4},
pages={1416-1429},
doi={10.1109/TIT.2007.892778},
ISSN={0018-9448},
month={April},}

@INPROCEEDINGS{gaudio2019performance,
author={L. {Gaudio} and M. {Kobayashi} and B. {Bissinger} and G. {Caire}},
booktitle={IEEE  ICC Workshops}, 
title={Performance Analysis of Joint Radar and Communication using OFDM and OTFS}, 
year={2019},
volume={},
number={},
pages={1-6},}

@INPROCEEDINGS{nimr2018extendedGFDM,
author={A. {Nimr} and M. {Chafii} and M. {Matthe} and G. {Fettweis}},
booktitle={IEEE_C_GC},
title={Extended {GFDM} Framework: {OTFS} and {GFDM} Comparison},
year={2018},
volume={},
number={},
pages={1-6},
doi={10.1109/GLOCOM.2018.8647704},
ISSN={2576-6813},
month={Dec},}

@INPROCEEDINGS{hadani2017otfs,
author={R. {Hadani} and S. {Rakib} and A. F. {Molisch} and C. {Ibars} and A. {Monk} and M. {Tsatsanis} and J. {Delfeld} and A. {Goldsmith} and R. {Calderbank}},
booktitle={2017 IEEE MTT-S International Microwave Symposium (IMS)},
title={Orthogonal Time Frequency Space ({OTFS}) modulation for millimeter-wave communications systems},
year={2017},
volume={},
number={},
pages={681-683},
doi={10.1109/MWSYM.2017.8058662},
ISSN={},
month={June},}

@INPROCEEDINGS{murali2018onOTFSmodulation,
author={K. R. {Murali} and A. {Chockalingam}},
booktitle={2018 Information Theory and Applications Workshop (ITA)},
title={On {OTFS} Modulation for High-Doppler Fading Channels},
year={2018},
volume={},
number={},
pages={1-10},
doi={10.1109/ITA.2018.8503182},
ISSN={},
month={Feb},}

@article{telatar1999capacity,
author = {Telatar, Emre},
title = {Capacity of Multi-antenna Gaussian Channels},
journal = EUROP_J_TTELE,
volume = {10},
number = {6},
pages = {585-595},
doi = {10.1002/ett.4460100604},
year = {1999}
}

@book{blahut1987principles,
  title={{Principles and practice of information theory}},
  author={Blahut, Richard E},
  volume={1},
  year={1987},
  publisher={Addison-Wesley Reading}
}



@ARTICLE{blahut1972computation,
  author={R. {Blahut}},
  journal=it, 
  title={Computation of channel capacity and rate-distortion functions}, 
  year={1972},
  volume={18},
  number={4},
  pages={460-473},
  doi={10.1109/TIT.1972.1054855}}



@article{cheng2019low,
  title={Low-Complexity Linear Equalizers for {OTFS} Exploiting Two-Dimensional Fast Fourier Transform},
  author={Cheng, Junqiang and Gao, Hui and Xu, Wenjun and Bie, Zhisong and Lu, Yueming},
  journal={arXiv preprint arXiv:1909.00524},
  year={2019}
}

@article{mahler2016tracking,
  title={Tracking of wideband multipath components in a vehicular communication scenario},
  author={Mahler, Kim and Keusgen, Wilhelm and Tufvesson, Fredrik and Zemen, Thomas and Caire, Giuseppe},
  journal=IEEE_J_VT,
  volume={66},
  number={1},
  pages={15--25},
  year={2016},
  publisher={IEEE}
}


@article{mahler2016measurement,
  title={Measurement-based wideband analysis of dynamic multipath propagation in vehicular communication scenarios},
  author={Mahler, Kim and Keusgen, Wilhelm and Tufvesson, Fredrik and Zemen, Thomas and Caire, Giuseppe},
  journal=IEEE_J_VT,
  volume={66},
  number={6},
  pages={4657--4667},
  year={2016},
  publisher={IEEE}
}

@ARTICLE{raviteja2019OTFSchannelEst,
author={P. {Raviteja} and K. T. {Phan} and Y. {Hong}},
journal=IEEE_J_VT,
title={{Embedded Pilot-Aided Channel Estimation for OTFS in Delay-Doppler Channels}},
year={2019},
volume={68},
number={5},
pages={4906-4917},
month={May}
}

@inproceedings{cordeiro2010ieee,
  title={{IEEE} 802.11 ad: Introduction and performance evaluation of the first multi-Gbps {WiFi} technology},
  author={Cordeiro, Carlos and Akhmetov, Dmitry and Park, Minyoung},
  booktitle={Proceedings of the 2010 ACM international workshop on mmWave communications: from circuits to networks},
  pages={3--8},
  year={2010},
  organization={ACM}
}

@ARTICLE{boutros2002multiuserDecoding,
author={J. {Boutros} and G. {Caire}},
journal=IEEE_J_IT,
title={Iterative multiuser joint decoding: unified framework and asymptotic analysis},
year={2002},
volume={48},
number={7},
pages={1772-1793},
keywords={iterative decoding;multiuser channels;code division multiple access;graph theory;interference suppression;approximation theory;Gaussian processes;binary codes;convolutional codes;interleaved codes;trellis codes;error statistics;iterative multiuser joint decoding;asymptotic analysis;code-division multiple-access;CDMA signals;factor-graph representation;sum-product algorithm;parallel interference cancellation algorithm;serial interference cancellation algorithm;hard interference cancellation algorithm;soft interference cancellation algorithm;asymptotic performance;code block length;density evolution;random spreading;large-system limit;Gaussian approximation;decoder soft output;stable fixed points;one-dimensional nonlinear dynamical system;1D nonlinear dynamical system;binary convolutional codes;bit-interleaving;multiuser detection;BER analysis;M-PSK trellis codes;Code division multiaccess;Graph theory;Interference suppression;Approximation methods;Gaussian processes;Convolutional codes;Interleaved coding;Trellis codes;Error analysis},
doi={10.1109/TIT.2002.1013125},
ISSN={},
month={July},}

@ARTICLE{Richardson2001capacity,
author={T. J. {Richardson} and R. L. {Urbanke}},
journal=IEEE_J_IT ,
title={The capacity of low-density parity-check codes under message-passing decoding},
year={2001},
volume={47},
number={2},
pages={599-618},
keywords={error detection codes;turbo codes;memoryless systems;telecommunication channels;error statistics;concatenated codes;iterative decoding;low-density parity-check codes;code capacity;message-passing decoding;binary-input memoryless channel;continuous output alphabet;discrete output alphabet;error probability;code length;outer code;code rate;decoder performance;binary-symmetric channel;binary message-passing algorithm;belief-propagation decoders;turbo codes;concatenated coding;iterative decoding;Error detection coding},
doi={10.1109/18.910577},
ISSN={},
month={Feb},}

@ARTICLE{wang1999interference,
author={ {Xiaodong Wang} and H. V. {Poor}},
journal=IEEE_J_COM,
title={Iterative (turbo) soft interference cancellation and decoding for coded {CDMA}},
year={1999},
volume={47},
number={7},
pages={1046-1061},
keywords={intersymbol interference;computational complexity;interference suppression;code division multiple access;iterative decoding;turbo codes;telecommunication network reliability;receivers;convolutional codes;multipath channels;channel coding;least mean squares methods;iterative soft interference cancellation;coded CDMA;multiple-access interference;intersymbol interference;reliable communications;multipath code-division multiple-access;iterative receiver structure;multiuser information data;convolutionally coded asynchronous multipath DS-CDMA system;soft-output decisions;soft-input soft-output;iterative process;a priori information;turbo decoding;multipath CDMA channel;sliding-window SISO multiuser detector;computational complexity;low-complexity SISO multiuser detector;nonlinear interference suppression technique;soft interference cancellation;instantaneous linear minimum mean-square error filtering;recursive implementation;signal-to-noise ratio;Interference cancellation;Iterative decoding;Intersymbol interference;Multiaccess communication;Multiple access interference;Detectors;Interference suppression;Impedance;Convolutional codes;Convolution},
doi={10.1109/26.774855},
ISSN={},
month={July},}

@INPROCEEDINGS{zhang2018channelEstOTFScs,
author={M. {Zhang} and F. {Wang} and X. {Yuan} and L. {Chen}},
booktitle={2018 IEEE International Conference on Communication Systems (ICCS)},
title={2{D} Structured Turbo Compressed Sensing for Channel Estimation in {OTFS} Systems},
year={2018},
volume={},
number={},
pages={45-49},
keywords={channel estimation;compressed sensing;delays;least mean squares methods;Markov processes;radio networks;time-varying channels;two-dimensional structured minimum mean-square error estimator;Markov random field;OTFS systems;high-speed mobility;wireless communications;orthogonal frequency-division multiplexing;accurate Doppler compensation;orthogonal time frequency space;time-frequency domain;clustered sparsity;channel information;fast time-varying channel estimation;two-dimensional delay-Doppler domain;two-dimensional structured turbo compressed sensing algorithm;2D structured turbo compressed sensing;channel estimation;compressed sensing;message passing;OTFS;structured sparsity},
doi={10.1109/ICCS.2018.8689234},
ISSN={},
month={Dec},}

@ARTICLE{Kschischang2001SPA,
author={F. R. {Kschischang} and B. J. {Frey} and H. -. {Loeliger}},
journal=IEEE_J_IT,
title={Factor graphs and the sum-product algorithm},
year={2001},
volume={47},
number={2},
pages={498-519},
keywords={graph theory;message passing;functional analysis;artificial intelligence;signal processing;digital communication;iterative decoding;Viterbi decoding;belief networks;Kalman filters;fast Fourier transforms;hidden Markov models;turbo codes;sum-product algorithm;factor graphs;global functions;local functions;factorization;bipartite graph;generic message-passing algorithm;computational rule;marginal functions;global function;artificial intelligence;signal processing;digital communications;forward/backward algorithm;Viterbi algorithm;iterative turbo decoding algorithm;belief propagation algorithm;Bayesian networks;Kalman filter;fast Fourier transform;FFT algorithms;HMM;Graph theory},
doi={10.1109/18.910572},
ISSN={},
month={Feb},}

@article{fuhrmann1992cfar,
  title={A {CFAR} adaptive matched filter detector},
  author={Fuhrmann, Daniel R and Kelly, Edward J and Nitzberg, Ramon},
  journal=IEEE_J_AES,
  volume={28},
  number={1},
  pages={208--216},
  year={1992}
}

@article{hakobyan2019high,
  title={High-performance automotive radar: A review of signal processing algorithms and modulation schemes},
  author={Hakobyan, Gor and Yang, Bin},
  journal=IEEE_M_SP,
  volume={36},
  number={5},
  pages={32--44},
  year={2019},
  publisher={IEEE}
}

@ARTICLE{song2019BeamAlignment,
	author={X. {Song} and S. {Haghighatshoar} and G. {Caire}},
	journal=IEEE_J_WCOM,
	title={Efficient Beam Alignment for Millimeter Wave Single-Carrier Systems With Hybrid {MIMO} Transceivers},
	year={2019},
	volume={18},
	number={3},
	pages={1518-1533},
	keywords={array signal processing;channel estimation;direction-of-arrival estimation;least squares approximations;millimetre wave communication;MIMO communication;multipath channels;radio transceivers;channel model parameters;fast channel variations;multipath components;beamformed channel;single-carrier communication;millimeter wave single-carrier systems;hybrid MIMO transceivers;millimeter wave bands;signal-to-noise ratio;beam alignment problem;single-carrier mm-wave communications;pre-specified pseudorandom beamforming codebook;pseudorandom spreading codes;angle-of-arrival/angle-of-departure pair;multipath channel;mm-wave channels;AoA-AoD domain;nonnegative vector;nonnegative least squares technique;strongest AoA-AoD pair;propagation channel;next generation wireless networks;Channel estimation;Array signal processing;Doppler shift;Signal to noise ratio;Delays;OFDM;Wireless communication;mm-wave;beam alignment;single-carrier communications;multipath channels;compressed sensing;nonnegative least squares (NNLS)},
	doi={10.1109/TWC.2019.2892043},
ISSN={1558-2248},
month={March},}

@INPROCEEDINGS{muns2019beamAlignment,
	author={G. R. {Muns} and K. V. {Mishra} and C. B. {Guerra} and Y. C. {Eldar} and K. R. {Chowdhury}},
	booktitle={IEEE INFOCOM 2019 - IEEE Conference on Computer Communications Workshops (INFOCOM WKSHPS)},
	title={Beam Alignment and Tracking for Autonomous Vehicular Communication using {IEEE} 802.11ad-based Radar},
	year={2019},
	volume={},
	number={},
	pages={535-540},
	keywords={array signal processing;millimetre wave communication;mobility management (mobile radio);protocols;road vehicle radar;telecommunication network routing;wireless LAN;vehicular traffic;in-band radar;beam alignment;autonomous vehicular communication;roadside base stations;millimeter wave bands;off-the-shelf IEEE 802.11ad WiFi router;radar functionality;beam tracking;millimeter wave band;IEEE 802.11ad-based radar;IEEE 802.11ad protocol;frequency 60.0 GHz;Doppler radar;Doppler effect;Training;Radar tracking;Throughput;Data transfer;IEEE 802.11ad;mmWave;automotive radar;beam alignment;CAV},
	doi={10.1109/INFCOMW.2019.8845121},
	ISSN={null},
	month={April},}

@ARTICLE{grossi2018opportunisticRadar,
	author={E. {Grossi} and M. {Lops} and L. {Venturino} and A. {Zappone}},
	journal=IEEE_J_SP,
	title={Opportunistic Radar in  {IEEE} 802.11ad Networks},
	year={2018},
	volume={66},
	number={9},
	pages={2441-2454},
	keywords={array signal processing;probability;radar detection;wireless LAN;opportunistic radar;IEEE 802.11ad networks;probing signal;sector level sweep;prospective obstacles;radial velocity;signal amplitude;prior information;channel fluctuation;Cramér-Rao;observation window;numerical examples;detection probability;size 90.0 m;size 10.0 cm;Radar;Standards;Array signal processing;Protocols;Training;Bandwidth;Receivers;Opportunistic radar;Cramér-Rao bound;generalized likelihood ratio test;mmWaves;60 GHz;IEEE 802.11ad},
	doi={10.1109/TSP.2018.2813300},
	ISSN={1941-0476},
	month={May},}

@article{grossi2019adaptive,
	title={{Adaptive detection and localization exploiting the IEEE 802.11 ad standard}},
	author={Grossi, Emanuele and Lops, Marco and Venturino, Luca},
	journal={arXiv preprint arXiv:1904.12835},
	year={2019}
}

@INPROCEEDINGS{dokhanchi2018ofdmJRC,
	author={S. H. {Dokhanchi} and M. R. B. {Shankar} and T. {Stifter} and B. {Ottersten}},
	booktitle={2018 IEEE Radar Conference (RadarConf18)},
	title={{OFDM}-based automotive joint radar-communication system},
	year={2018},
	volume={},
	number={},
	pages={0902-0907},
	keywords={iterative methods;mobile communication;OFDM modulation;parameter estimation;road vehicle radar;radar parameter estimation;automotive joint radar-communication system;radar processing;receiver processing;iterative estimation;communication link;range estimation;OFDM;OFDM;Receivers;Doppler effect;Radar cross-sections;Estimation;Doppler radar;Radar-Communication system;Alternating Least Square (ALS);orthogonal frequency division multiplex­ing (OFDM);spatial diversity;space-time processing;array-processing},
	doi={10.1109/RADAR.2018.8378680},
	ISSN={2375-5318},
	month={April},}

@book{vitetta2013wireless,
  title={Wireless communications: algorithmic techniques},
  author={Vitetta, Giorgio A and Taylor, Desmond P and Colavolpe, Giulio and Pancaldi, Fabrizio and Martin, Philippa A},
  year={2013},
  publisher={John Wiley \& Sons},
}


@book{el2011network,
  title={Network Information Theory},
  author={A.{El Gamal} and Y.{H. Kim}},
  year={2011},
  publisher={Cambridge University Press},
}


@article{gaudio2020jointMimoOTFS,
  title={Joint Radar Target Detection and Parameter Estimation with MIMO OTFS},
  author={Gaudio, Lorenzo and Kobayashi, Mari and Caire, Giuseppe and Colavolpe, Giulio},
  journal={arXiv preprint arXiv:2004.11035},
  year={2020}
}


%\bibliography{estcomm}
@ARTICLE{choudhuri2013causal,
  author={C. {Choudhuri} and Y. {Kim} and U. {Mitra}},
  journal=it, 
  title={Causal State Communication}, 
  year={2013},
  volume={59},
  number={6},
  pages={3709-3719},
  doi={10.1109/TIT.2013.2245719}
  }
  

